MOREA: a GPU-accelerated Evolutionary Algorithm for Multi-Objective Deformable Registration of 3D Medical Images

Finding a realistic deformation that transforms one image into another, in case large deformations are required, is considered a key challenge in medical image analysis. Having a proper image registration approach to achieve this could unleash a number of applications requiring information to be transferred between images. Clinical adoption is currently hampered by many existing methods requiring extensive configuration effort before each use, or not being able to (realistically) capture large deformations. A recent multi-objective approach that uses the Multi-Objective Real-Valued Gene-pool Optimal Mixing Evolutionary Algorithm (MO-RV-GOMEA) and a dual-dynamic mesh transformation model has shown promise, exposing the trade-offs inherent to image registration problems and modeling large deformations in 2D. This work builds on this promise and introduces MOREA: the first evolutionary algorithm-based multi-objective approach to deformable registration of 3D images capable of tackling large deformations. MOREA includes a 3D biomechanical mesh model for physical plausibility and is fully GPU-accelerated. We compare MOREA to two state-of-the-art approaches on abdominal CT scans of 4 cervical cancer patients, with the latter two approaches configured for the best results per patient. Without requiring per-patient configuration, MOREA significantly outperforms these approaches on 3 of the 4 patients that represent the most difficult cases.

==> figures/tex/results/ct-resolutions.tex <==
\begin{table}[H]
    \centering
    \begin{tabularx}{\linewidth}{lXr}
        \toprule
        Patient & Scan & In-slice Resolution \\
        \midrule
        \multirow{2}{*}{Patient 1} & Full bladder & $(0.86,0.86)$\emph{mm}\\
        & Empty bladder & $(0.98,0.98)$\emph{mm} \\
        
        \midrule
        \multirow{2}{*}{Patient 2} & Full bladder & $(1.04,1.04)$\emph{mm}\\
        & Empty bladder & $(1.07,1.07)$\emph{mm} \\
        
        \midrule
        \multirow{2}{*}{Patient 3} & Full bladder & $(0.98,0.98)$\emph{mm}\\
        & Empty bladder & $(0.98,0.98)$\emph{mm} \\
        
        \midrule
        \multirow{2}{*}{Patient 4} & Full bladder & $(1.04,1.04)$\emph{mm}\\
        & Empty bladder & $(1.00,1.00)$\emph{mm} \\
        \bottomrule
    \end{tabularx}
    \vspace{0.05cm}
    \caption{In-slice resolutions for the slices of each CT scan, prior to resampling them to $(1.5,1.5)$\emph{mm}.}
    \label{tab:ct-resolutions}
    \vspace{-0.4cm}
\end{table}


==> figures/tex/results/landmark-reference.tex <==
\begin{table}[H]
    \centering
    \begin{tabularx}{\linewidth}{Xlr}
        \toprule
        Identifier & Description & Baseline Error \\
        \midrule
        \texttt{ext\_anal\_sfinct} & External anal sphincter & 2.3\emph{mm}\\
        \texttt{cervix\_os} & Cervical ostium & 3.4\emph{mm} \\
        \texttt{int\_urethral\_os} & Internal urethral ostium & 3.3\emph{mm}\\
        \texttt{ext\_urethral\_os} & External urethral ostium & 3.4\emph{mm}\\
        \texttt{ureteral\_os\_right} & Ureteral ostium right & 5.3\emph{mm}\\
        \texttt{ureteral\_os\_left} & Ureteral ostium left & 12.0\emph{mm}\\
        \texttt{int\_anal\_sfinct} & Internal anal sphincter & 3.7\emph{mm}\\
        \bottomrule
    \end{tabularx}
    \vspace{0.05cm}
    \caption{Landmarks used in the evaluation of registrations and their baseline registration errors after rigid registration.}
    \label{tab:landmarks}
    \vspace{-0.4cm}
\end{table}


==> figures/tex/results/significance-full.tex <==
%\multirow{2}{*}{Patient 2}
\begin{table}
    \centering
    \begin{tabularx}{\linewidth}{Xlrr}
        \toprule
        Problem & Contour & MOREA / Elastix & MOREA / ANTs \\
        \midrule
\multirow{7}{*}{Patient 1} 
& bladder & \textbf{0.011} (+) & \textbf{0.007} (+)\\
& bones & \textbf{0.009} (+) & \textbf{0.006} (+)\\
& rectum & \textbf{0.007} (+) & \textbf{0.007} (+)\\
& anal canal & \textbf{0.007} (+) & \textbf{0.007} (+)\\
& sigmoid & \textbf{0.007} (+) & \textbf{0.007} (+)\\
& bowel & \textbf{0.010} (+) & \textbf{0.011} (+)\\
& body & \textbf{0.006} (+) & \textbf{0.006} (-)\\
\midrule

\multirow{7}{*}{Patient 2} 
& bladder & \textbf{0.007} (+) & \textbf{0.007} (+)\\
& bones & \textbf{0.007} (+) & \textbf{0.007} (+)\\
& rectum & 0.118 (+) & \textbf{0.007} (-)\\
& anal canal & 0.123 (-) & 0.180 (-)\\
& sigmoid & \textbf{0.007} (+) & \textbf{0.007} (-)\\
& bowel & 0.401 (+) & \textbf{0.007} (+)\\
& body & 0.655 (+) & 1.000 (-)\\
\midrule

\multirow{7}{*}{Patient 3} 
& bladder & \textbf{0.012} (+) & \textbf{0.007} (+)\\
& bones & \textbf{0.007} (+) & \textbf{0.007} (+)\\
& rectum & 0.290 (+) & \textbf{0.007} (-)\\
& anal canal & 0.118 (-) & \textbf{0.007} (+)\\
& sigmoid & \textbf{0.007} (+) & \textbf{0.007} (+)\\
& bowel & \textbf{0.007} (+) & 0.056 (+)\\
& body & \textbf{0.007} (+) & 0.118 (+)\\
\midrule

\multirow{7}{*}{Patient 4} 
& bladder & \textbf{0.007} (+) & 0.195 (-)\\
& bones & \textbf{0.007} (-) & \textbf{0.007} (-)\\
& rectum & \textbf{0.010} (-) & \textbf{0.007} (-)\\
& anal canal & 0.606 (+) & \textbf{0.007} (-)\\
& sigmoid & \textbf{0.009} (+) & 0.118 (+)\\
& bowel & 0.119 (+) & 0.119 (-)\\
& body & \textbf{0.020} (-) & \textbf{0.020} (-)\\
        \bottomrule
    \end{tabularx}
    \vspace{0.05cm}
    \caption{\textbf{p}-values of pair-wise comparisons of Hausdorff distances for all contours between approaches, computed by the two-sided Mann-Whitney U test. A plus (\texttt{+}) indicates a better mean with MOREA, a minus (\texttt{-}) the opposite. Significant results are highlighted according to a Bonferroni-corrected $\alpha$ of 2.5\%.}
    \label{tab:significance-full}
    \vspace{-0.4cm}
\end{table}


==> figures/tex/results/tres.tex <==
\begin{table}[t]
    \centering
    \begin{tabularx}{\linewidth}{Xrrrr}
        \toprule
        Problem & Baseline & Elastix & ANTs & MOREA \\
        \midrule
Patient 1 & 4.8 $\pm$ 3.1 & 5.6 $\pm$ 2.8 & 4.2 $\pm$ 2.0 & 4.8 $\pm$ 2.0\\
Patient 2 & 7.5 $\pm$ 4.0 & 11.8 $\pm$ 7.3 & 7.7 $\pm$ 4.3 & 7.8 $\pm$ 3.8\\
Patient 3 & 9.5 $\pm$ 6.7 & 6.4 $\pm$ 2.0 & 7.7 $\pm$ 2.6 & 6.5 $\pm$ 1.9\\
Patient 4 & 14.1 $\pm$ 9.5 & 8.1 $\pm$ 4.3 & 6.3 $\pm$ 3.4 & 6.8 $\pm$ 4.0\\
        \bottomrule
    \end{tabularx}
    \vspace{0.05cm}
    \caption{Target registration errors (mean and standard deviation) for the shown registrations of each approach on each patient, across repeats. All errors are specified in \emph{mm}.}
    \label{tab:tres}
    \vspace{-0.4cm}
\end{table}


==> sup/figures/tex/results/landmark-reference.tex <==
\begin{table}[H]
    \centering
    \begin{tabularx}{\linewidth}{Xlr}
        \toprule
        Identifier & Description & Baseline Error \\
        \midrule
        \texttt{ext\_anal\_sfinct} & External anal sphincter & 2.3\emph{mm}\\
        \texttt{cervix\_os} & Cervical ostium & 3.4\emph{mm} \\
        \texttt{int\_urethral\_os} & Internal urethral ostium & 3.3\emph{mm}\\
        \texttt{ext\_urethral\_os} & External urethral ostium & 3.4\emph{mm}\\
        \texttt{ureteral\_os\_right} & Ureteral ostium right & 5.3\emph{mm}\\
        \texttt{ureteral\_os\_left} & Ureteral ostium left & 12.0\emph{mm}\\
        \texttt{int\_anal\_sfinct} & Internal anal sphincter & 3.7\emph{mm}\\
        \bottomrule
    \end{tabularx}
    \vspace{0.05cm}
    \caption{Landmarks used in the evaluation of registrations and their baseline registration errors after rigid registration.}
    \label{tab:landmarks}
    \vspace{-0.4cm}
\end{table}


==> sup/figures/tex/results/metric-comparison-plot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{sup/figures/plots/comparisons/603/hausdorff.pdf}
    \caption{Hausdorff distances for solutions produced by compared approaches on Patient~1.}
    \label{fig:comparison:metric-plot}
    \vspace{-0.4cm}
\end{figure}

